A spectral element solution of the Poisson equation with shifted boundary polynomial corrections: influence of the surrogate to true boundary mapping and an asymptotically preserving Robin formulation

We present a new high-order accurate spectral element solution to the two-dimensional scalar Poisson equation subject to a general Robin boundary condition. The solution is based on a simplified version of the shifted boundary method employing a continuous arbitrary order $hp$-Galerkin spectral element method as the numerical discretization procedure. The simplification relies on a polynomial correction to avoid explicitly evaluating high-order partial derivatives from the Taylor series expansion, which traditionally have been used within the shifted boundary method. In this setting, we apply an extrapolation and novel interpolation approach to project the basis functions from the true domain onto the approximate surrogate domain. The resulting solution provides a method that naturally incorporates curved geometrical features of the domain, overcomes complex and cumbersome mesh generation, and avoids problems with small-cut-cells. Dirichlet, Neumann, and general Robin boundary conditions are enforced weakly through: i) a generalized Nitsche's method and ii) a generalized Aubin's method. For this, a consistent asymptotic preserving formulation of the embedded Robin formulations is presented. We present several numerical experiments and analysis of the algorithmic properties of the different weak formulations. With this, we include convergence studies under polynomial, $p$, increase of the basis functions, mesh, $h$, refinement, and matrix conditioning to highlight the spectral and algebraic convergence features, respectively. This is done to assess the influence of errors across variational formulations, polynomial order, mesh size, and mappings between the true and surrogate boundaries.

==> Texts/Old_texts/Discussion.tex <==
\section{Discussion}\label{sec:discussion}

In this section, we discuss and highlight different findings from the numerical results. First, we discuss results from Dirichlet boundary conditions on a weak symmetrical formulation. Secondly, the observed irregularities within the interpolating SBM procedures are discussed.

\subsection{Dirichlet boundary conditions on symmetrical forms}

For the results presented in the previous section, only non-symmetrical bi-linear forms were considered as presented in Section \ref{sec:mathematical_problem}. The associated symmetrical forms for Dirichlet boundary conditions are listed in Appendix \ref{sec:appendix_symmetric}. Similar analyses have been performed for the symmetrical forms with a close-to or identical agreement for the CBM, SBM-ei, and SBM-i. Regarding the SBM-e, the ill-conditioning problem was intensified by multiple orders of magnitude, where larger polynomial orders yield the most prominent difference when comparing the symmetric and non-symmetric formulations. The explanation hereof follows the one highlighted in Section \ref{sec:numerical_method_and_discretization}, namely the unbounded polynomial nature of the nodal Lagrange basis outside the elements. The symmetrized terms require the extrapolated basis functions to be squared, which only enhances the ill-conditioning of the Vandermonde matrix and, ultimately, the entire linear system. For $P=1$, non to minor discrepancies are detected. 




\subsection{Irregularities when interpolating}



As noticed throughout Section \ref{sec:numerical_results}, some irregularities within the matrix-conditioning are present when using the interpolation approaches (SBM-ei and SBM-i). To gain some insights into this numerical phenomenon, we propose a small one-dimensional analysis. We define a standard reference domain, $\mathcal{R} = \{r | r \geq -1 ; r \leq 1 \}$, on ${\rm I\!R}^{1}$ for the polynomial basis. Given some polynomial order, $P$, and associated Gauss-Lobatto quadrature points in $\mathcal{R}$, we can define a well-behaved and well-conditioned Vandermonde matrix, $\mathcal{V}$, for interpolation within the reference domain. Next, we consider the right-most point in $\mathcal{R}$ denoted by $r_{\text{r}}$, that attain the coordinate value of $r_{\text{r}} = 1$. From this, we define a shifted point, $r_{\text{s}}$, that either can be inside or outside the element by shifting $ r_{\text{r}}$ with $r^* \in [-2;2]$, such that $r_{\text{s}} = r_{\text{r}} + r^* = 1 + r^*$. From this, we have that
\begin{itemize}
    \item $r^* = 0$ implies that $r_{\text{s}} = r_{\text{r}}$.
    \item $r^* < 0$ implies an interpolating point within $\mathcal{R}$, where $r^* = -2$ correspond to $r_{\text{s}}$ being located at the left-most point in the reference domain.
    \item $r^* > 0$ implies an extrapolation point outside $\mathcal{R}$ to the right of $r _{\text{r}}$.
\end{itemize}

A concept illustration of this is given in Figure \ref{fig:V_test}.

\begin{figure}[h]
    \vspace{7mm}
    \centering
    \vspace{7mm}
    \includegraphics{Figures/V_test.eps}
    \caption{Illustration of the one-dimensional domain for the simple interpolation/extrapolation analysis.}
    \label{fig:V_test}
\end{figure}

Using this definition, the study of interpolation and extrapolation in terms of $\kappa(\mathcal{V})$ can be studied by moving $r_{\text{s}}$ with $r^* \in [-2;2]$. In Figure \ref{fig:Test_1D_cond_V}, the results are shown for different polynomial orders, $P \leq 9$. First, it is observed how extrapolation results in the continuous growth of the condition number as we increase $r^*$, which also gets enhanced for increasing $P$ as seen in Figure \ref{fig:circle_within_circle}, e.g., for $P=1$, $\kappa(\mathcal{V})|_{r^*=2} \approx 4 \cdot 10^0$ and for $P = 10$, $\kappa(\mathcal{V})|_{r^*=2} \approx 3 \cdot 10^7$. Secondly, concerning interpolation, it is noted how certain locations in $\mathcal{R}$ -- the quadrature points -- provide an increased condition number. In practice, this corresponds to placing two nodes in the same location. Also, the neighborhood around the quadrature points intensifies the ill-conditioning, whereas points between two quadrature points provide a local minimum. This observation implies that one should be intelligent about the nodal placement in interpolation mode, which is entirely achievable with the SBM through the mapping, $\mathcal{M}$. An idea could be to incorporate an efficient and simple optimization strategy with the aim of minimizing the matrix conditioning on an element basis to -- hopefully -- further improve the overall conditioning of the method. In principle, further analysis should be carried out for this numerical phenomenon, especially in two dimensions. Lastly, it is evident from the figure at the higher polynomial order, the more favorable -- on average -- interpolation is over extrapolation.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.95]{Figures/Test_1D_cond_V.eps}
    \caption{Conditioning of the Vandermonde matrix, $\kappa(\mathcal{V})$, in interpolation and extrapolation for various polynomial orders, $P \leq 9$. Interpolation (full blue), extrapolation (full red), quadrature points in $\mathcal{R}$ (dashed black).}
    \label{fig:Test_1D_cond_V}
\end{figure}


% \subsection{Comparing to quadrilateral elements} 

==> Texts/Old_texts/Results.tex <==
\section{Numerical Results}\label{sec:numerical_results}
In the following, we discuss a considerable number of experiments (for Dirichlet, Neumann, and Robin problems), most of which run on meshes composed of triangular elements that are quasi-uniform in size and arranged in an unstructured manner, e.g., the ones of Figure \ref{fig:three_mappings}. We will consider finite elements of polynomial degree up to $P=10$ on meshes generated using the open-source meshing software Gmsh \cite{Geuzaine2009}. An essential input to Gmsh is a characteristic length, $l_c$, that is an approximate size of the desired elements. In Figure \ref{fig:three_mappings}, a characteristic length of $l_c = 0.25$ is used to mesh a circle with radius $R = 0.375$ for SBM-e, SBM-ei, and SBM-i. Meshes for the two latter will be identical and differ from the former, generally with fewer elements for the same $l_c$, e.g., see Table \ref{tab:three_meshes_info}. In general, test examples of a circle with radius $R$ are considered unless otherwise stated. Also, the proposed model is currently implemented in Matlab, version R2022a, and the linear system of equations in \eqref{eq:linear_system_of_equations} is solved directly within this framework.

For simplicity, we use the same exact solution throughout the paper, obtained with the classical method of manufactured solutions (MMS). This provides controlled analytical definitions for the boundary conditions and forcing terms. These are derived based on a pre-assumed true solution, $u_{\text{MMS}}(x,y)$. We construct the solution to the Poisson problem, such that $u_{\text{MMS}}(x,y) \in C^{\infty}$, by combining trigonometric functions with a linear polynomial twist as
\begin{equation}
    u_{\text{MMS}}(x,y) = \cos \left ( \frac{x\pi}{L_x} \right )  \sin \left ( \frac{y\pi}{L_y} \right ) + 2x - 1y,
\end{equation}
where $L_x = 1$ and $L_y = 1$ are the domain lengths in the $x$ and $y$-directions, respectively. As an error measure, we exploit exact global integration through the SEM on the affine elements, with this $\|u_{\text{MMS}} - u_{\text{SEM}} \|_{L^1} = \int_{\Omega} |u_{\text{MMS}} - u_{\text{SEM}} | d \Omega$.

\underline{\textit{Outline of results}}:
The results will be presented in the following way: First, we compare Nitsche's to Aubin's method for the pure Dirichlet problem. Secondly, we verify our implementation (again, for the pure Dirichlet problem) on \textit{well-behaved} meshes, namely meshes in which the surrogate boundary is purposely parallel to a conformal discretization of the true boundary. This numerical experiment aims to -- qualitatively -- compare with other high-order SBM implementations in the literature. Next, we turn to unstructured meshes (for Dirichlet, Neumann, and Robin problems) as these kinds of meshes are the more natural choice of meshing, despite the fact that the convergence rates and conditioning are highly dependent on the unstructuredness of the discrete representation. We investigate the importance of the mapping between the surrogate and true boundaries and the use of the Robin formulations as a general boundary condition to impose all boundary conditions within a single implementation and a variable Robin coefficient, $\varepsilon$. Lastly, we provide a quantitative overall assessment of the implemented solver for multiple mesh configurations at the end of this section.



\subsection{Dirichlet boundary conditions -- On well-behaved meshes}\label{sec:DBC_on_nice_meshes}





\subsubsection{\JV{Comparing Nitsche's to Aubin's method}}

\JV{\textit{Comment by JV: Here, we present results for DBC on nice meshes. We consider CBM and SBM-e. I would say that $p$-convergence is enough. So actually, the plots that I show in "small report". Conclusion is that we can get better conditioning and convergence for high-order using Aubin's method. Then, in the following, we only use this method. @Mario, what do you think?}}

% \JV{As an initial investigation,...}
% \JV{This conclusion is supported by multiple numerical experiences (not shown)}


\subsubsection{\emph{h}-convergence and conditioning}


Before investigating the properties of the schemes on unstructured meshes, we verify our implementation in the Dirichlet case for a well-behaved case. With this, $\Gamma_N \cup \Gamma_R = \emptyset$. We purposely align the surrogate boundary to the true one, such that $\overline{\boldsymbol{n}} \cdot \boldsymbol{n} \approx 1$. To do so, we consider a true domain as a circle of radius $R = 0.375$, and generate the unfitted mesh by fitting another circle of radius $R \pm l_c/4$. Obviously, the cases with "$+$" are for interpolation modes (SBM-ei and SBM-i), whereas "$-$" is for the extrapolation mode (SBM-e). Meshes for CBM are constructed trivially. \JV{We solely consider Aubin's method; however, close-to-identical results have been obtained for Nitsche's approach in convergence yet with larger condition numbers for SBM-e, SBM-ei, and SBM-i}. We choose the penalty constant to be $\tau = \frac{2}{h_{\text{avg}}}$, as this in the CBM case has been seen to provide the expected algebraic convergence rates in general. We perform $h$-convergence error analysis and condition number analysis up to polynomial degrees $P \leq 5$, to attempt an indirect validation with respect to the results of \cite{Atallah2022,Collins2023}.

\begin{figure}[h]
    \centering
    \vspace{10mm}
    \includegraphics[scale = 0.9]{Figures/h_convergence_nice_mesh.eps}
    \caption{$h$-convergence (left column) and associated condition number study (right column) for $P \leq 5$ for Dirichlet boundary conditions for CBM, SBM-e, SBM-ei, and SBM-i on a \textit{well-behaved} mesh.}
    \label{fig:h_convergence_nice_mesh}
\end{figure}

The results are reported in Figure \ref{fig:h_convergence_nice_mesh}. As mentioned in all previous works, despite unfitted meshes, the shifted boundary approach provides genuinely high-order results with comparable errors. We can also see (visually) that -- up to $P=5$ -- the condition number obtained for all methods is comparable, with the SBM-e giving slightly higher values for increasing $P$. All the methods follow monotonically the $\mathcal{O}(1/h_{\max}^{2})$ scaling in conditioning as for the CBM approach. This is one of the key features of the SBM approach due to the complete absence of small cut cells. The numbers obtained -- in terms of magnitude and scaling -- are comparable to those presented, e.g., in \cite{Collins2023}. Concerning the error convergence, the SBM-e, which is classically used in previous SBM works, is comparable to the others for $P=1$ and $P=2$ (perhaps slightly better). However, the SBM-ei and SBM-i give smaller errors for $P \ge 3$. All these results align with those presented in \cite{Atallah2022,Collins2023} and confirm the potential of the SBM strategy. 









\subsubsection{The effect of extrapolation}

The use of the interpolation approaches, SBM-ei and SBM-i, should be motivated. Therefore, we wish to study extrapolation's effect in the SBM-e setting numerically. Consider the setup and visualization shown in Figure \ref{fig:circle_within_circle_visualization}, where a circle of radius $R=0.375$ initially is meshed conformally with $l_c = 0.15$ resulting in $N_{\text{elm}}=64$ elements. Then, the distance between the true boundary, $\Gamma$, and the surrogate boundary, $\overline{\Gamma}$, is varied as $d(\boldsymbol{\overline{x}}) = l_c \cdot a$, with $a = [0.01;2]$. Hereby, $a=0.01$ will essentially result in a close-to-conformal method, and as $a$ increases, the basis functions are extrapolated further. We note that $a \geq 0.5$ is essentially a violation of the classical SBM as the two boundaries will no longer be in the neighborhood of each other.

\begin{figure}[t]
    \centering
\includegraphics{Figures/circle_within_circle_visualization.eps}
    \caption{Visualization of meshing setup for the numerical study of the extrapolation effect with SBM-e for high orders. Initial conformal mesh of a circle with radius $R=0.375$. The distance, $d(\overline{\boldsymbol{x}})$, between $\Gamma$ (red line) and $\overline{\Gamma}$ (outer-most blue lines). For the mesh $l_c = 0.15$ and $N_{\text{elm}} = 64$.}
    \label{fig:circle_within_circle_visualization}
\end{figure}

The numerical results are presented in Figure \ref{fig:circle_within_circle} for error convergence and conditioning of the system matrix, $\kappa(\mathcal{A})$, under the increase of polynomial order, $P$, when increasing the distance between the two boundaries, $d(\boldsymbol{\overline{x}})$. From the figure, it is observed that increasing $d(\boldsymbol{\overline{x}})$ will increase the matrix conditioning in a spectral (exponential) fashion, which can especially be seen for large, $P$. The increase in $\kappa(\mathcal{A})$ effects the $p$-convergence by decreasing the exponential rate of convergence, but also -- at some point (e.g., $P=9$) -- ruins the rate of decay, as the problem becomes too ill-conditioned. The decrease in convergence rate is also because the true circle is enlarged as the distance increase. With this, the boundary data from $\Gamma$ is distributed more scattered across the boundary, which makes the solution less resolved. It can be noted that the close-to-conformal case drives the numerical error down to machine accuracy, where round-off errors start to accumulate. For $P=1$, it is observed that the effect of extrapolation is more or less uninfluenced for $d(\boldsymbol{\overline{x}}) \leq l_c \cdot 0.5$. 

\begin{figure}[t]
    \centering
\includegraphics{Figures/circle_within_circle.eps}
    \caption{Left: $p$-convergence study with Dirichlet boundary conditions for SBM-e with the numerical setup as shown in Figure \ref{fig:circle_within_circle_visualization}.
Right: Associated study of the matrix conditioning, $\kappa(\mathcal{A})$, for the same setup.}
    \label{fig:circle_within_circle}
\end{figure}

The reasonable explanation of the exponential increase in matrix conditioning partly stems from the natural behavior of the nodal basis functions, i.e., the Lagrange polynomials, $h(x,y)$, as outlined in Section \ref{sec:SEM} and discussed in Section \ref{sec:note_on_conditioning}. Inside the element, the polynomials attain a maximum absolute function value of $\max |h(x,y)| = 1$ at the nodal mesh points; however, the polynomials grow unbounded outside the element. This growth only amplifies for higher polynomial orders. The consequence of extrapolation can also be studied by considering the conditioning of the Vandermonde matrix, $\kappa(\mathcal{V})$, for interpolation and/or extrapolation. Recall from Section \ref{sec:numerical_method_and_discretization} that the original nodal placement was of Gauss-Lobatto-type such that the Lebesque constant was minimized and thereby ensuring a well-behaved Vandermonde matrix for interpolation. Now, in the SBM context, this feature is -- to a large extent -- violated. For pure extrapolation, $\kappa(\mathcal{V})$, grows exponentially under $P$ increase, and at more rapid rates when increasing the extrapolation distance. This motivates using the SBM-ei and the SBM-i, where the nodal placement is almost or entirely inside the element. We will now evaluate the different choices (SBM-e, SBM-ie, and SBM-i) in a more general and natural meshing setting.








\subsection{Dirichlet boundary conditions -- On unstructured meshes} 

\subsubsection{\emph{p}-convergence and conditioning}

For the $p$-convergence study, we consider two meshes for each solution approach (CBM, SBM-e, SBM-ei, and SBM-i), namely $l_c = 0.15$ and $l_c = 0.05$. The number of elements, $N_{\text{elm}}$, and the average edge lengths, $h_{\text{avg}}$ are listed in Table \ref{tab:three_meshes_info}. The table shows that $h_{\text{avg}} \approx l_c$. As expected, the SBM-e will yield fewer elements than SBM-ei and SBM-i. This difference feature will become less pronounced as the mesh is refined. Lastly, it can be noted that the meshes of SBM-ei and SBM-i are identical.

\begin{table}[h]
    \centering
    \caption{For CBM, SBM-e, SBM-ei, and SBM-i: Number of elements and average edge length for the two meshes ($l_c = 0.15$ and $l_c = 0.05$) as: $N_{\text{elm}} ~(h_{\text{avg}})$.}
    \begin{tabular}{l l l l l} 
    \toprule
        $l_c$ & CBM & SBM-e & SBM-ei & SBM-i  \\ \midrule
       $0.15$ & 64 (0.1264) & 35 (0.1421) & 73 (0.1424) & 73 (0.1424) \\
       $0.05$ & 450 (0.0477) & 357 (0.0500) & 462 (0.0499) & 462 (0.0499) \\
       \bottomrule
    \end{tabular}
    \label{tab:three_meshes_info}
\end{table}

The results of the $p$-convergence study -- where we keep the mesh fixed and vary the polynomial order of the expansions -- on the two different meshes can be seen in the left plot in Figure \ref{fig:P_convergence_non_sym_DBC}. For the CBM, it is evident that the error converges for the two meshes in the norm, ultimately reaching machine precision around $10^{-15}$, where the rate of spectral convergence is more rapid on the finer mesh (an early indication of algebraic convergence). Hereafter, round-off errors start to accumulate. The spectral convergent behaviors for SBM-ei and SBM-i are fairly similar and reach a level of $\approx 10^{-14}$ at $P=7$ and $P=9$ for the fine and coarser mesh, respectively, and the accuracy follows the one of the CBM. Lastly, the SBM-e converges at a slower rate than the aforementioned three approaches, e.g., for $l_c = 0.05$ and $P=7$, a difference of 2-3 orders in magnitude is seen, and for $l_c = 0.15$ and $P=8$, about 2 orders of magnitude in difference is observed. This difference is less pronounced for low order, i.e., $P \leq 2$. As was also observed in Figure \ref{fig:circle_within_circle}, the rate of convergence is ruined at some point ($P \approx 7$ and $P\approx9$ for the fine and coarse meshes, respectively), which is a consequence of ill-conditioning of the system.

Regarding conditioning on the right plot of Figure \ref{fig:P_convergence_non_sym_DBC}, the four approaches are similar for low orders, yet, as the polynomial order increases, the CBM yields the best-conditioned system. The conditioning is worse for the SBM-ei and the SBM-i, e.g., about 2-3 orders of magnitude for $P=10$ compared to the CBM. From the analysis of these two meshes, SBM-ei seems better conditioned than SBM-i for $P \leq 5$ and vice versa for $P>5$. It can be noted that a certain level of irregularity is observed in the condition number for SBM-ei, e.g., for $P = 9$. This mesh-dependent irregularity is highlighted and discussed in Section \ref{sec:overall_assessment}. Lastly, the SBM-e is -- by far -- the most ill-conditioned system of the four approaches, which explains the aforementioned ruining of the convergence rates.

\begin{figure}[t]
    \centering \includegraphics{Figures/P_convergence_non_sym_DBC.eps}
    \caption{Left: $p$-convergence study with Dirichlet boundary conditions for the CBM, SBM-e, SBM-ei, and SBM-i for two different meshes: $l_c = 0.15$ (full lines) and $l_c = 0.05$ (dashed lines). Right: Associated study of the matrix conditioning, $\kappa(\mathcal{A})$, for the same numerical setup.}
    \label{fig:P_convergence_non_sym_DBC}
\end{figure}




\subsubsection{\emph{h}-convergence and conditioning}

To complete the convergence study, we now consider what happens when fixing the polynomial order, $P$, and then decreasing the size of the elements. This $h$-convergence study is shown in Figure \ref{fig:h_convergence_non_sym_DBC} for $P \leq 9$. From the figure, it is confirmed that the algebraic order of convergence is $\mathcal{O}(h_{\max}^{P+1})$ for the CBM, SBM-e, SBM-ei, and SBM-i. Note that for high orders, e.g., $P \geq 6$, the errors of those three approaches are near -- or have reached -- machine accuracy; thus, round-off errors start to dominate. Regarding SBM-e, the expected order of convergence can be confirmed for $P \leq 6$, whereas for $P > 6$, the convergence is ruined. Comparing the three SBM approaches, it can be concluded that for $P=1$, the SBM-e looks to provide lower errors than SBM-ei and SBM-i; however, for $P \geq 2$, the two interpolating strategies are superior to the classical extrapolating one (1-2 orders of magnitude for $P \in [2;6]$). There is a similar agreement between SBM-ei and SBM-i throughout the analysis, yet, for high orders ($P \geq 8$), the error for the latter is slightly smaller. 



Figure \ref{fig:h_convergence_non_sym_DBC_cond_A} displays the matrix conditioning study of the $h$-convergence analysis. From this, it is seen that the algebraic growth rate of the condition number is second-order independent of the polynomial order. Concerning SBM-e, it is evident that $\kappa(\mathcal{A})$ grows rapidly for higher orders, especially when the mesh is too coarse for a particular polynomial order. Comparing SBM-ei and SBM-i, it is observed that the latter yields the best-conditioned system of the two for $P \geq 6$, which agrees with the conclusion from the $p$-convergence study. It should be noted that the conditioning for the highest orders behaves slightly irregularly, as pointed out within the $p$-convergence study. See the overall assessment of the three SBM approaches in Section \ref{sec:overall_assessment} and the $h$-convergence study on a well-behaved mesh in Section \ref{sec:DBC_on_nice_meshes}. In general, the results on conditioning for $P=1$ and $P=2$ agree in magnitude and rate with results presented in \cite{Main2018a,Nouveau2019}.

\begin{figure}[h]
    \centering
    \vspace{10mm}
    \includegraphics[scale = 0.9]{Figures/h_convergence_non_sym_DBC.eps}
    \caption{$h$-convergence study for $P \leq 9$ for Dirichlet boundary conditions for CBM, SBM-e, SBM-ei, and SBM-i.}
    \label{fig:h_convergence_non_sym_DBC}
\end{figure}

\begin{figure}[h]
    \centering
    \vspace{10mm}
    \includegraphics[scale = 0.9]{Figures/h_convergence_non_sym_DBC_cond_A.eps}
    \caption{Study of matrix conditioning under $h$-refinement for $P \leq 9$ for Dirichlet boundary conditions for CBM, SBM-e, SBM-ei, and SBM-i. System matrices are from the study in Figure \ref{fig:h_convergence_non_sym_DBC}.}
    \label{fig:h_convergence_non_sym_DBC_cond_A}
\end{figure}





\newpage ~ \\
\newpage ~ \\
\newpage 







\subsection{Neumann boundary conditions -- On unstructured meshes} 

Next, we consider Neumann boundary conditions such that $\Gamma_D \cup \Gamma_R = \emptyset$. For the studies, we again consider Aubin's formulation; however, this one is identical to the one of Nitsche. For conciseness, the figures for the Neumann problem are placed in Appendix \ref{sec:appendix_neumann}.

\subsubsection{\emph{p}-convergence and conditioning}

For the $p$-convergence, we use the exact same setup as for the Dirichlet conditions on unstructured meshes, namely two meshes ($l_c = 0.15$ and $l_c = 0.05$) for the CBM, SBM-e, SBM-ei, and SBM-i as given in Table \ref{tab:three_meshes_info}. The study results are shown in Figure \ref{fig:P_convergence_non_sym_NBC} with $p$-convergence to the left and the associated matrix conditioning to the right. Concerning the CBM, the errors converge to machine precision for both meshes, with the finest reaching this level at $P = 7$ and the coarsest at $P = 9$. In this study, the SBM-i can be observed to converge at a similar rate as SBM-ei; however, with about 1 order of magnitude lower in accuracy for $P \geq 4$. At $P = 10$, the convergence rate for SBM-ei seems to be ruined. Before this, both interpolating approaches reach a precision level of about $10^{-13}$. No ruining of convergence can be seen for SBM-i besides the accumulation of round-off errors. For the SBM-e, the convergence rate on both meshes is lower than the other SBM procedures, and the convergent behavior gets ruined at some point, as in the Dirichlet case.

%%

Regarding conditioning, the CBM is -- as expected -- the lowest of the four. For $P \leq 3$, SBM-ei and SBM-i are much alike; however, for $P > 3$, the latter seems to provide the smallest condition number (about 2 orders of magnitude for $P=10$). Some irregularity in SBM-ei is again observed here (see $P =4$ and $P=9$). Comparing $\kappa(\mathcal{A})$ for SBM-e from Figure \ref{fig:P_convergence_non_sym_DBC} with the one from Figure \ref{fig:P_convergence_non_sym_NBC}, an increase in condition number of about 3 orders of magnitude can be observed. The explanation is primarily related to the fact that when imposing Neumann boundary conditions, gradients in the basis functions are required. The SEM basis functions are now well-defined inside the elements and grow rapidly and unbounded outside the element; hence, the gradients will enhance this polynomial behavior even more outside the element. Ultimately, this will imply a worsening of the matrix conditioning. In general, SBM-e provides much larger $\kappa(\mathcal{A})$ than SBM-ei and SBM-i. Lastly, the irregularities in $\kappa(\mathcal{A})$ are spotted again.


\subsubsection{\emph{h}-convergence and conditioning}

The $h$-convergence studies for fixed polynomial order of $P \leq 9$ are shown in Figure \ref{fig:h_convergence_non_sym_NBC}. We generally confirm $\mathcal{O}(h_{\max}^P)$ convergence rate for the SBM-e, SBM-ei, and SBM-i, and $\mathcal{O}(h_{\max}^{P+1})$ for the CBM. This reduction in accuracy compared to the CBM is a known artifact of employing the Taylor series expansions in connection with the polynomial correction. The SBM-e provides the right convergence rate for $P \leq 6$. Compared to the SBM-ei and the SBM-i, the three approaches are fairly similar for $P=1$, then for $P \geq 2$, the two interpolating procedures are superior, e.g., between 1-3 orders of magnitude. The SBM-ei and the SBM-i follow each other; however, with a slightly favorable accuracy for the latter, especially for $P \geq 7$, which corresponds well with the SBM-ei having an extrapolating component. Thus the procedure is prone to having its convergence rate ruined at some order with some mesh configurations. We stress the mesh-related influence on convergence and condition as will be assessed in Section \ref{sec:overall_assessment}.

%% 

The associated matrix conditioning results obtained for the $h$-convergence studies are shown in Figure \ref{fig:h_convergence_non_sym_NBC_cond_A}. As seen before, the general growth rate for $\kappa(\mathcal{A})$ is second order. For $P = 1$, all approaches agree in conditioning; however, a clear difference is observed for higher orders. For $P \leq 3$, SBM-ei and the SBM-i are close to identical in magnitude, yet, for $P \geq 4$, the latter system is better conditioned. The CBM provides the overall best-conditioned system for $P \geq 2$. The reduction in accuracy order when exploiting the polynomial correction $P=1$ seems to be an infeasible choice for the SBM approaches due to potentially ill-conditioning for large systems, i.e., first-order accurate and second-order conditioning.

%%














\subsection{Robin boundary conditions -- On unstructured meshes}

Lastly, Robin boundary conditions are considered for Aubin's method, such that $\Gamma_D \cup \Gamma_N = \emptyset$. This numerical study ensures that the formulation collapses to the essential and natural boundary conditions for various $\varepsilon$. We do so by choosing three different values of $\varepsilon$: i) low ($\varepsilon = 10^{-5}$), ii) medium ($\varepsilon = 10^{0}$), and iii) high ($\varepsilon = 10^{5}$). Then, for a particular mesh ($l_c = 0.05$), we study the familiar $p$-convergence and associated condition number for the CBM and the SBM-i. Note that the Robin penalty constant is set to equal the Dirichlet penalty term, $1/\gamma = \tau = 2/h_{\text{avg}}$, and to ensure well-posedness in the limit when $\varepsilon^{-1} \xrightarrow{} 0$, we impose a single Dirichlet point condition in the middle of the domain as done for the pure Neumann condition.

In Figure \ref{fig:P_convergence_RBC_CBM} and Figure \ref{fig:P_convergence_RBC_SBM_i}, the results with the CBM and the SBM-i are shown, respectively. It can be confirmed for both implementations that the Robin condition collapses to a Dirichlet condition for a low value of $\varepsilon$, and similarly to a Neumann condition for a high value of $\varepsilon$. For the medium value, a mix -- both in terms of convergence and conditioning -- is achieved as expected. Minor discrepancies are evident between the Dirichlet and Robin conditions results with low $\varepsilon$. This difference is due to the enforcement of the single Dirichlet point condition. As a final remark, various other meshes have undergone similar tests, ultimately yielding identical -- or close to identical -- results. 

\begin{figure}[h]
    \centering
    \includegraphics{Figures/P_convergence_RBC_CBM.eps}
    \caption{For the CBM on mesh a with $l_c = 0.05$: $p$-convergence and associated matrix conditioning, $\kappa(\mathcal{A})$, for Robin boundary conditions with three different values of $\varepsilon = \{10^{-5}, 10^0, 10^{5}\}$. Comparison with pure Dirichlet and Neumann results from Figure \ref{fig:P_convergence_non_sym_DBC} and Figure \ref{fig:P_convergence_non_sym_NBC}, respectively.}
    \label{fig:P_convergence_RBC_CBM}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics{Figures/P_convergence_RBC_SBM_i.eps}
    \caption{For the SBM-i on a mesh with $l_c = 0.05$: $p$-convergence and associated matrix conditioning, $\kappa(\mathcal{A})$, for Robin boundary conditions with three different values of $\varepsilon = \{10^{-5}, 10^0, 10^{5}\}$. Comparison with pure Dirichlet and Neumann results from Figure \ref{fig:P_convergence_non_sym_DBC} and Figure \ref{fig:P_convergence_non_sym_NBC}, respectively.}
    \label{fig:P_convergence_RBC_SBM_i}
\end{figure}










\subsubsection{\JV{One or two analyses on the RBC}}
\JV{@Mario, what should be include here? See slack for some of the plots.}







%
%\newpage ~ \\
%\newpage ~ \\
%\newpage ~ \\
\newpage


\subsection{Overall assessment of the three SBM approaches}\label{sec:overall_assessment} % Overall assessment of SBM approaches:

Throughout this numerical results section, we have seen various solutions with the three SBM approaches. As noted, some irregularities were present occasionally. Those irregularities are due to mesh sensitivity, i.e., where and how the true domain is placed on the surrogate domain. For example, consider the SBM-e and imagine a mesh where all elements -- luckily -- are placed such that the method resembles the one of a CBM. On the other hand, the elements could also have been placed in an  unlucky manner with a large distance between $\Gamma$ and $\overline{\Gamma}$. Due to this, the convergence rates are not always perfectly monotonic, as seen multiple times in SBM literature \cite{Nouveau2019,Collins2023}. Therefore, we wish to compare SBM-e, SBM-ei, and SBM-i more quantitatively to justify whether the interpolating approaches improve the numerical scheme over the classical extrapolation approach.

We consider a $(L_x \times L_y)$ square domain, with $L_x = L_y = 2$, that is meshed using $l_c = 0.15$ quasi-uniformly distributed triangular elements. Now, 100 circles of radius $R =0.375$ are embedded into the background mesh (one at a time) given a randomly generated center as shown in Figure \ref{fig:Overall_assessment_mesh}. For each of the 100 mesh configurations, we consider the classical $p$-convergence studies and conditioning for Dirichlet boundary conditions (Figure \ref{fig:Overall_assessment_DBC_Convergence_non_sym} and Figure \ref{fig:Overall_assessment_DBC_Conditioning_non_sym}, respectively) and Neumann boundary conditions (Figure \ref{fig:Overall_assessment_NBC_Convergence_non_sym} and Figure \ref{fig:Overall_assessment_NBC_Conditioning_non_sym}, respectively) in a box-plot fashion. The median and variance of the order of magnitude, $\log_{10}(\cdot)$, of the error in $p$-convergence and conditioning are listed in Table \ref{tab:overall_assessment_convergence} and Table \ref{tab:overall_assessment_conditioning}, respectively. The results are considered below in three groups, namely $P = 1$ (first order), $ 1 < P \leq 5$ (medium to high orders), and $5 > P \leq 10$ (very high orders).

\begin{figure}[h]
    \centering
    \includegraphics{Figures/Overall_assessment_mesh.eps}
    \caption{Mesh visualization for overall assessment. 100 circles of radius $R = 0.375$ with randomly generated centers. Highlighted center in red and all centers in blue. Moreover, $l_c = 0.15$. }
    \label{fig:Overall_assessment_mesh}
\end{figure}

\underline{\textit{First order:}} For $P = 1$, the results generally show that all three SBM approaches are alike regarding median and variance. The only deviating result is for the error considering Dirichlet boundary conditions. Here, the SBM-e provides a slightly smaller error (0.5 order of magnitude). Compared with \cite{Main2018a,Nouveau2019}, a similar size of the condition number for SBM-e can be seen. 

\underline{\textit{Medium to high orders:}} For $ 1 < P \leq 5$, an improvement can be observed using SBM-ei or SBM-i over SBM-e, especially towards the higher polynomial orders. A significant difference can be spotted at $P = 5$ for $\kappa(\mathcal{A})$, i.e., around 4 orders of magnitude for Dirichlet and 3-4 for Neumann. Compared with Collins et al. \cite{Collins2023}, similar sizes of the condition numbers for SBM-e can be seen. When we compare SBM-ei and SBM-i, little to no improvements can be seen for Dirichlet boundary conditions, whereas some differences can be observed for Neumann in favor of the latter. However, this difference is between 0.5 to 1 order of magnitude for $P = 5$ and insignificant for $P \leq 3$.


\underline{\textit{Very high orders:}} Now, for $5 < P \leq 10$, the reduction in conditioning is considerable by choosing SBM-ei or SBM-i over SBM-e. As much as 9 orders of magnitude for the Neumann boundary condition using $P = 10$ can be gained. In general, the SBM-i provides the lowest median with the smallest variance compared to the SBM-ei. Regarding convergence, recall that the convergence rate for $P > 5$ using SBM-e is highly influenced by ill-conditioning; hence, it is not fair to compare against. 

\begin{table}[h]
    \centering
    \caption{Median and variance of $\log_{10}(\|u_{\text{MMS}} - u_{\text{SEM}} \|_{L^1})$ for the 100 different circle positions for SBM-e, SBM-ei, and SBM-i. Results for both Dirichlet and Neumann cases.}
    \begin{tabular}{r c c c c c c c c c c} \toprule
   $P$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & $10$ \\ \midrule
   
        Dirichlet -- median: & & & & & & & & & & \\ \midrule
        SBM-e & -2.4 &  -3   & -3.9 & -4.6 & -5.7 & -6.5 & -7.7 & -8.9  & -9.1  & -7.7  \\
        SBM-ei & -2   & -3.2 & -4.5 & -5.8 & -7.3 & -8.4 & -9.9 & -11.2 & -12.4 & -12   \\
        SBM-i & -1.9 & -3.1 & -4.4 & -5.8 & -7.2 & -8.6 & -9.9 & -11.4 & -12.6 & -12.3 \\ \midrule
        
        Dirichlet -- variance: & & & & & & & & & & \\ \midrule
         SBM-e &   0.02 & 0.03 & 0.03 & 0.05 & 0.10 & 0.21 & 0.38 & 0.15 & 0.98 & 1.23 \\
        SBM-ei &  0.01 & 0.02 & 0.01 & 0.03 & 0.02 & 0.25 & 0.23 & 0.27 & 0.34 & 0.61 \\
        SBM-i &  0.01 & 0.02 & 0.01 & 0.03 & 0.02 & 0.06 & 0.10 & 0.18 & 0.21 & 0.30 \\ \midrule
        
         Neumann -- median: & & & & & & & & & & \\ \midrule
         SBM-e & -1.2 & -1.4 & -2.4 & -3   & -4   & -4.9 & -6.1 & -7.2  & -6.7  & -5.4  \\
         SBM-ei & -1.2 & -1.8 & -3.5 & -4.6 & -5.4 & -6.9 & -8.4 & -10.3 & -11.5 & -11   \\
         SBM-i & -1.2 & -1.8 & -3.4 & -4.4 & -6.3 & -7.4 & -9.1 & -10.5 & -11.9 & -11.9 \\  \midrule

        Neumann -- variance: & & & & & & & & & & \\ \midrule
        SBM-e &  0.10 & 0.28 & 0.13 & 0.29 & 0.39 & 0.38 & 0.29 & 0.35 & 1.87 & 1.55 \\
          SBM-ei &   0.08 & 0.21 & 0.15 & 0.38 & 0.69 & 0.56 & 0.65 & 0.68 & 0.89 & 0.76 \\
          SBM-i &   0.08 & 0.21 & 0.19 & 0.37 & 0.49 & 0.43 & 0.42 & 0.59 & 0.69 & 0.82\\ 

         \bottomrule
    \end{tabular}
    \label{tab:overall_assessment_convergence}
\end{table}


\begin{table}[h]
    \centering
    \caption{Median and variance of $\log_{10}(\kappa(\mathcal{A}))$ for the 100 different circle positions for SBM-e, SBM-ei, and SBM-i. Results for both Dirichlet and Neumann cases.}
    \begin{tabular}{r c c c c c c c c c c} \toprule
   $P$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ & $9$ & $10$ \\ \midrule
   
        Dirichlet -- median: & & & & & & & & & & \\ \midrule
       SBM-e & 1.2 & 2.4 & 3.2 & 6.1 & 8   & 10.1 & 11.4 & 12.2 & 13.6 & 15.3 \\
       SBM-ei & 1.3 & 2   & 2.5 & 3.4 & 4   & 5.3  & 5.8  & 6.8  & 7.6  & 8.6  \\
        SBM-i & 1.3 & 2   & 2.7 & 3.6 & 4.3 & 4.8  & 5.6  & 6.5  & 7.2  & 7.9  \\ \midrule
        
        Dirichlet -- variance: & & & & & & & & & & \\ \midrule
       SBM-e & 0.00 & 0.04 & 0.03 & 0.99 & 1.58 & 2.70 & 2.86 & 1.95 & 2.21 & 1.90 \\
       SBM-ei & 0.00 & 0.00 & 0.01 & 0.03 & 0.08 & 0.54 & 0.42 & 0.55 & 0.58 & 0.86 \\
       SBM-i & 0.00 & 0.00 & 0.01 & 0.05 & 0.11 & 0.10 & 0.16 & 0.25 & 0.31 & 0.35 \\ \midrule
       
         Neumann -- median: & & & & & & & & & & \\ \midrule
          SBM-e & 2.5 & 3.8 & 5.1 & 7.7 & 9.4 & 11.4 & 12.8 & 14.1 & 15.7 & 17.1 \\
         SBM-ei & 2.6 & 3.7 & 4.2 & 5.2 & 6.3 & 7    & 7.7  & 8.1  & 8.7  & 9.6  \\
         SBM-i & 2.6 & 3.6 & 4.1 & 4.7 & 5.3 & 5.7  & 6.5  & 7.2  & 7.7  & 8.3  \\  \midrule

  Neumann -- variance: & & & & & & & & & & \\ \midrule
      SBM-e &   0.01 & 0.22 & 0.19 & 1.27 & 2.32 & 2.80 & 2.25 & 1.87 & 2.49 & 1.53 \\
    SBM-ei & 0.02 & 0.04 & 0.11 & 0.38 & 0.75 & 0.65 & 0.96 & 0.84 & 0.98 & 1.03 \\
    SBM-i & 0.02 & 0.04 & 0.12 & 0.16 & 0.42 & 0.28 & 0.44 & 0.50 & 0.68 & 0.86 \\ 

    \bottomrule
     
    \end{tabular}
    \label{tab:overall_assessment_conditioning}
\end{table}

\begin{figure}[h]
    \centering
     \vspace{5mm}
    \includegraphics[scale = 0.9]{Figures/Overall_assessment_DBC_Convergence_non_sym.eps}
    \caption{Box-plot: Overall assessment $p$-convergence for Dirichlet boundary condition according to mesh in Figure \ref{fig:Overall_assessment_mesh} in box-plot format for SBM-e, SBM-ei, and SBM-i. Black dots are the median.}
\label{fig:Overall_assessment_DBC_Convergence_non_sym}
\end{figure}

\begin{figure}[h]
    \centering
    \vspace{5mm}
    \includegraphics[scale = 0.9]{Figures/Overall_assessment_DBC_Conditioning_non_sym.eps}
    \caption{Box-plot: Overall assessment of $\kappa(\mathcal{A})$ for study in Figure \ref{fig:Overall_assessment_DBC_Convergence_non_sym}. Black dots are the median.}
\label{fig:Overall_assessment_DBC_Conditioning_non_sym}
\end{figure}

\begin{figure}[h]
    \centering
    \vspace{5mm}
    \includegraphics[scale = 0.9]{Figures/Overall_assessment_NBC_Convergence_non_sym.eps}
    \caption{Box-plot: Overall assessment $p$-convergence for Neumann boundary condition according to mesh in Figure \ref{fig:Overall_assessment_mesh} in box-plot format for SBM-e, SBM-ei, and SBM-i. Black dots are the median.}
\label{fig:Overall_assessment_NBC_Convergence_non_sym}
\end{figure}

\begin{figure}[h]
    \centering
    \vspace{5mm}
    \includegraphics[scale = 0.9]{Figures/Overall_assessment_NBC_Conditioning_non_sym.eps}
    \caption{Box-plot: Overall assessment of $\kappa(\mathcal{A})$ for study in Figure \ref{fig:Overall_assessment_NBC_Convergence_non_sym}. Black dots are the median.}
\label{fig:Overall_assessment_NBC_Conditioning_non_sym}
\end{figure}


\newpage ~ \\
\newpage ~  \\
\newpage 

==> ToDo.tex <==
\textbf{To-Do-List (from Mario):} \textit{Please @Mario, please delete if item is checked off}

\begin{itemize}
\item {\color{red}\bf STATEMENT: We aim at constructing an embedded discrete Robin formulation which}
\begin{enumerate}
\item \textit{All BCs in one formulation}: degenerates correctly to  Neumann or Dirichlet  for $\varepsilon=0$ or 
$\varepsilon^{-1}=0$
\item for $\varepsilon$ or 
$\varepsilon^{-1}$ very small but non null, is asymptotically consistent with the continuous equations
\item It is arbitrarily high order with the smallest possible condition numbers
\end{enumerate}
\item  {\color{red}\bf FINDING: what   impacts the above objecive:}
\begin{enumerate}
\item definition of the surrogate domain (mapping and extrapolation/interpolation)
\item variational form (e.g. Niche vs Aubin's penalty)
\end{enumerate}
\item {\color{red}\bf Theory: add section recalling the penalty method} after the  Nitche method. Justification: from numerical evidence related to  the CN  for $p\ge 5$
\item {\color{red}\bf Theory: add section on generalized penalty method (or penalty-Robin method) } after the generlized Nitche method. Justification: from numerical evidence related to  the CN  for $p\ge 5$

\item {\color{red}\bf Theory: add AP analysis for the  generalized penalty method (or penalty-Robin method) }

\item {\color{red}\bf Theory: add section on embedded generalized penalty method (or penalty-Robin method) with AP analysis } 

% \item {\bf Figure 1: missing a conformal mesh ?} \JV{Done, see Figure \ref{fig:computational_domains}.}

% \item  {\bf add table with lebesgue constants (inside and outside the element)  !} : e.g. mirroring the element wrt each edge !!!!! \JV{Done, see Table \ref{tab:Lebesque_constants} and Figure \ref{fig:Lebesque_constants}.}

% \item {\bf more accent on Robin :  e.g. add statistics study for medium case  (the others we assume give the same as Dirichled and Neumann)} \JV{Is this not that same (ish) at the bullet below (about asymptotic consistency)?}

% \item \textbf{maybe remove some results using pure Diriclet and Neumann ?} \JV{I've moved the NBC result plots to the appendix. Should be good.}

% \item {\bf  add a test using Robin+ mixed BCs with different $\varepsilon$ values on $\Gamma$.} \JV{I think we should do this for the FNPF paper instead (It already works with the RBCs as a general \textit{two-in-one} BC in this solver). If I should make it work for the current triangular model, I would spend some time coding. I would much rather spend my time elsewhere at the moment.}

% \item {\bf not so sure about what to think of section 8... I'm wondering if we shouldn't leave this for future, or for the revision ;P...  } \JV{I've commented this sections out. This "numerical phenomenon" is actually every important. Take for example a periodic linear wave in interpolation mode. If we get unlucky, the solution will start to explode due to ill-conditioning.}

\item {\bf add a proof with $\varepsilon$ variable in space ? } not before september, but it's actually easy.. could be added during revision actually ! \JV{Do you want to add this now or after Revision \#1?}

\item verify numerically the asymptotic consistency (removing num. solution of m-1 order and study the convergence of the remainder wrt exact m order)  ???? VERY important but either for the revision of before journal submission. \JV{To understand you correctly (in a numerical setting): Using MMS, construct a true solution that is polynomial of some order $m$. And check that error drops to machine precision for $P \geq m$? I already did this back in Bordeaux with Mirco :) }

\item add comment on non-symmetric variant (what would be the asymtptic behaviour  for that ? add a corollary or remark to the propositions )
normally all is ok but maybe leave this  for the revision of before journal submission if we submit after summer. \JV{Have you thought more about this?}

\item stability for the Robin condition : can it be proved ????  maybe leave this alone. \JV{Mario, if you want to add this, please do so. That is up to you :)}
\end{itemize}


\textbf{To-Do-List (Mario):}
\begin{itemize}
\item in section 2: clarify the necessity of splitting the RHS. reason 1: numerical. reason 2: have the small perturbations of Dirichlet AND Neumann in
\item recall the  above clarification in the AP sections (theoretical at least)
and remove the appropriate term in the AP proofs
\end{itemize}

\textbf{FINAL To-Do-List:}
\begin{itemize}

\item (1) \MR{Mario}: Finish draft of the introduction. \JV{Jens}/\AP{Allan}: Once done, read and make corrections.
\item (1) \JV{Jens}: Finish the draft of the results section. \MR{Mario}/\AP{Allan}: Once done, read and make corrections.

\item (1) \MR{Mario}: See you other items above.

\item (2)  Write a new conclusion, a new abstract, and a new "paper aim and contributions".

\item (3) \textbf{All}: One more "start-to-finish" read.

\item (4) \JV{Jens:} Once done (and everything looks nice), submit to arXiv and BIT Journal.

\end{itemize}

\newpage

\tableofcontents
\newpage

